Improve Efficiency of Doubly Robust Estimator when Propensity Score is Misspecified

Doubly robust (DR) estimation is a crucial technique in causal inference and missing data problems. We propose a novel Propensity score Augmentved Doubly robust (PAD) estimator to enhance the commonly used DR estimator for average treatment effect on the treated (ATT), or equivalently, the mean of the outcome under covariate shift. Our proposed estimator attains a lower asymptotic variance than the conventional DR estimator when the propensity score (PS) model is misspecified and the outcome regression (OR) model is correct while maintaining the double robustness property that it is valid when either the PS or OR model is correct. These are realized by introducing some properly calibrated adjustment covariates to linearly augment the PS model and solving a restricted weighted least square (RWLS) problem to minimize the variance of the augmented estimator. Both the asymptotic analysis and simulation studies demonstrate that PAD can significantly reduce the estimation variance compared to the standard DR estimator when the PS model is wrong and the OR is correct, and maintain close performance to DR when the PS model is correct. We further applied our method to study the effects of eligibility for 401(k) plan on the improvement of net total financial assets using data from the Survey of Income and Program Participation of 1991.

==> archive.tex <==
\section{}
There exists approaches to improve the (intrinsic) efficiency of the doubly robust estimators when the PS is correctly specified and the OR is misspecified \citep{cao2009improving,tan2010bounded,rotnitzky2012improved}. While improving the efficiency when the PS is wrong and the OR is correct still remains to be an open problem. To handle this problem, we first inspect the asymptotic expansion of $\muhat\subCB$ under this scenario. Heuristically, suppose that $\widehat\bgamma$ weakly converge to some $\bar\gamma$, then
\begin{align*}
\muhat\subCB-\mu_0=&\widehat\EE_{\Ssc}\exp(\X\trans\widehat\bgamma)(Y-\X\trans\balpha_0)+\widehat\EE_{\Tsc}\X\trans\balpha_0-\mu_0\\
=&\widehat\EE_{\Ssc}\exp(\X\trans\bar\bgamma)(Y-\X\trans\balpha_0)+\widehat\EE_{\Tsc}m(\X)-\mu_0+o_p(n^{-1/2}).
\end{align*}
Thus, to reduce $\Var(n^{1/2}\{\muhat\subCB-\mu_0\})$, one would be interested in reducing
\[
\Var_{\Ssc}\{\exp(\X\trans\bar\bgamma)(Y-\X\trans\balpha_0)\}=\int p_{\Ssc}(\x)q(y|\x)\{\exp(\x\trans\bar\bgamma)\}^2(Y-\X\trans\balpha_0)^2 d\x dy.
\]
In usual cases, this integral can be further written as
\[
\Var_{\Ssc}\{\exp(\X\trans\bar\bgamma)(Y-\X\trans\balpha_0)\}=\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)\}^2 v_{\bar \btheta}(\X),
\]
with some function $v_{\bar \btheta}(\X)\geq 0$, e.g. when $Y$ is binary (non-linear link function needed) or 
\[
Y=\X\trans\balpha_0+v^{1/2}(\X)\varepsilon,~~\mbox{where}~\varepsilon\perp\X~\mbox{and}~\EE\varepsilon^2=1.
\]
Inspired by this, we propose to augment the PS model with some $\bPsi\trans\bbeta$, where $\bPsi$ is constructed from some pre-specified basis function of $\X$ as will be introduced later. %Later, we will present the construction procedure of $\bPsi$. 
In specific, we define that
\[
r\subLAug(\X;\bbeta)=\exp(\X\trans\widehat\bgamma)+\bPsi\trans\bbeta,
\]
and consider the estimator
\[
\muhat\subLAug=\widehat\EE_{\Ssc}Y\{\exp(\X\trans\widehat\bgamma)+\bPsi\trans\bbeta\}.
\]
To ensure the double robustness property of $\muhat\subLAug$, we preserve the constraint in (\ref{equ:2.1.1}) on the augmented $r\subLAug$:
\[
\widehat\EE_{\Ssc}\X\{\exp(\X\trans\widehat\bgamma)+\bPsi\trans\bbeta\}=\widehat\EE_{\Tsc}\X,
\]
which is equivalent with: $\widehat\EE_{\Ssc}\X\bPsi\trans\bbeta=\bzero$ by (\ref{equ:2.1.1}). Under this constraint on $\bbeta$, we aim at minimizing the variance term
\[
V_{\mu}(\bbeta)=\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bbeta\}^2 v_{\btheta}(\X).
\]
These lead to solving for the restricted (weighted) least square problem (RWLS):
\begin{equation}
\bar\bbeta={\rm argmin}_{\bbeta}V_{\mu}(\bbeta),\quad\mbox{s.t.}\quad\EE_{\Ssc}\X\bPsi\trans\bbeta=\bzero.
\label{equ:2.2.1}
\end{equation}
With a similar spirit to the intrinsic efficient construction of the OR model \citep[e.g.]{tan2010bounded,rotnitzky2012improved}, when the PS is correctly specified, i.e. $r(\x)=\exp(\x\trans\bgamma_0)$ and $\bgamma_0=\bar\bgamma$, we need to ensure that $r_{PCA}(\X;\bbeta)\xrightarrow{p}\exp(\X\trans\bgamma_0)$, which is equivalent with $\bar\bbeta=\bzero$. To achieve this, we only need to guarantee that
\[
\bzero=\frac{\partial V_{\mu}(\bbeta)}{\partial\bbeta}\Big|_{\bbeta=\bzero}=\EE_{\Ssc}\bPsi\exp(\X\trans\bar\bgamma)v_{\bar \btheta}(\X)=\EE_{\Tsc}\bPsi v_{\bar \btheta}(\X),
\]
when the PS: $r(\x)=\exp(\x\trans\bar\bgamma)$ is correct. For any pre-specified basis function $\bPhi=\bphi(\X)$ of $\X$ (e.g. the natural spline of each feature), this is implied by centralizing $\bPhi$ (on $\Tsc$ and weighted by $v_{\bar \btheta}(\X)$) to construct:
\[
\bPsi=\bPhi-\frac{\EE_{\Tsc}\bPhi v_{\bar \btheta}(\X)}{\EE_{\Tsc}v_{\bar \btheta}(\X)}.
\]
Empirically, our proposed construction procedures are outlined as follows:
\begin{enumerate}
    \item Solve the estimating equations (\ref{equ:2.1.1}) to derive $\widehat\bgamma$.
    
    \item Estimate $v_{\bar \btheta}(\X)=\Var[Y\mid\X]$ by $v_{\widehat\btheta}(\X)$. Specify a basis function $\bPhi=\bphi(\X)$, and let $\bPsi=\bPhi-{\widehat\EE_{\Tsc}[\bPhi v_{\widehat\btheta}(\X)]}/{\widehat\EE_{\Tsc}v_{\widehat\btheta}(\X)}$.
    
    \item Solve the RWLS problem:
\begin{equation}
\widehat\bbeta={\rm argmin}_{\bbeta}\widehat\EE_{\Ssc}\{\exp(\X\trans\widehat\bgamma)+\bPsi\trans\bbeta\}^2 v_{\widehat\btheta}(\X),\quad\mbox{s.t.}\quad\widehat\EE_{\Ssc}\X\bPsi\trans\bbeta=\bzero.
\label{equ:2.2.2}
\end{equation}

\item Obtain the estimator
\[
\muhat\subLAug=\widehat\EE_{\Ssc}Y\{\exp(\X\trans\widehat\bgamma)+\bPsi\trans\widehat\bbeta\}.
\]

\end{enumerate}



When $Y$ is binary, we assume that $m(\x)=g(\X\trans\balpha)$ and we have the estimation equation $\widehat\EE_{\Ssc}S(\widehat\balpha)=\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\widehat\balpha)\}=\bzero$. We assume that $\widehat\balpha$ convergences to $\bar\balpha$. By using Taylor series expansion, we have that \[
\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\bar\balpha)\}+\widehat\EE_{\Ssc}\frac{\partial S(\balpha)}{\partial \balpha\trans}\bigg|_{\bar\alpha}(\widehat\balpha-\bar\balpha)+o_p(\|\widehat\balpha-\bar\balpha\|_2)=0
\]
and we have
\[
\widehat\balpha-\bar\balpha=-\widehat\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha\trans}\bigg|_{\bar\balpha}\bigg\}^{-1}\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\bar\balpha)\}
\]
Consider the basic doubly robust estimator $\widehat\mu_{dr}$ that
\[
\widehat\mu_{dr}=\widehat\EE_{\Ssc}\{Y-g(\X\trans\widehat\balpha)\}\exp(\X\trans\widehat\bgamma)+\widehat\EE_{\Tsc}g(\X\trans\widehat\balpha)
\]
When OR model is correctly specified, we have $\bar\balpha=\balpha_0$ and $\EE_{\Ssc}\{Y-g(\X\trans\balpha_0)\}=0$. And by central limit theorem, we have $\widehat\balpha-\bar\balpha=O_p(n^{-1/2})$. Consider $\widetilde\mu_{dr}$, where
\begin{align*}
   &\widetilde\mu_{dr}=\widehat\EE_{\Ssc}\{Y-g(\X\trans\balpha_0)\}\exp(\X\trans\bar\bgamma)+\widehat\EE_{\Tsc}g(\X\trans\balpha_0)
   \\
   &+\bigg\{\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\balpha_0}\bigg\}\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}^{-1}\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\balpha_0)\}
\end{align*}
 It is obvious that $\EE\widetilde\mu_{dr}=\mu_0$ and $\widehat\mu_{dr}-\widetilde\mu_{dr}=o_p(n^{-1/2})$, which is shown by
 \begin{align*}
     &\widehat\mu_{dr}-\widetilde\mu_{dr}=\widehat\EE_{\Ssc}\{Y-g(\X\trans\balpha_0)\}\exp(\X\trans\bar\bgamma)\X\trans(\widehat\bgamma-\bar\bgamma)
     \\
     &-\bigg\{\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}(\widehat\balpha-\bar\balpha)+o_p(n^{-1/2})
     \\
     &-\bigg\{\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}^{-1}\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\balpha_0)\}
 \end{align*}
 by using central limit theorem, 
 \[
 \widehat\EE_{\Ssc}\{Y-g(\X\trans\balpha_0)\}\exp(\X\trans\bar\bgamma)\X\trans(\widehat\bgamma-\bar\bgamma)=[\EE_{\Ssc}\{Y-g(\X\trans\balpha_0)\}\exp(\X\trans\bar\bgamma)\X\trans+O_p(n^{-1/2})](\widehat\bgamma-\bar\bgamma)=o_p(n^{-1/2})
 \]
 on the other hand,
 \begin{align*}
    &- \bigg\{\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}(\widehat\balpha-\bar\balpha)\\
    &=\bigg\{\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}\widehat\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha}\bigg|_{\bar\balpha}\bigg\}^{-1}\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\bar\balpha)\}\\
    &=\bigg\{\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}+O_p(n^{-1/2})\bigg\}\bigg[\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}^{-1}+O_p(n^{-1/2})\bigg]\EE_{\Ssc}\X\{Y-g(\X\trans\bar\balpha)\}
 \end{align*}
 Hence, we have that
 \begin{align*}
     &-\bigg\{\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}(\widehat\balpha-\bar\balpha)
     \\
     &-\bigg\{\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}^{-1}\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\balpha_0)\}
     \\
     &=\widehat\EE_{\Ssc}\X\{Y-g(\X\trans\balpha_0)\}O_p(n^{-1/2})=o_p(n^{-1/2})
 \end{align*}
 Similar to the circumstance of linear model, we consider the augment estimator 
 \[
 \widehat\mu_{aug}=\widehat\EE_{\Ssc}\{Y-g(\X\trans\widehat\balpha)\}\{\exp(\X\trans\widehat\bgamma)+\widehat\bPsi\trans\widehat\bbeta\}+\widehat\EE_{\Tsc}g(\X\trans\widehat\balpha)
 \]
 and assume $\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}|_{\bar\balpha}\bPsi\trans\bbeta=\bzero$. Hence, when consider the variance of $n^{1/2}(\widehat\mu_{dr}-\mu_0)$, one may consider about the 
 \[
 \EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)\}^2 v_{\bar\btheta}(\X)+2l \EE_{\Ssc}\X\exp(\X\trans\bar\bgamma)v_{\bar \btheta}(\X)
 \]
where $l=\bigg\{\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\exp(\X\trans\bar\bgamma)-\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha}\bigg|_{\balpha_0}\bigg\}^{-1}$. For $ \widehat\mu_{aug}$, we are interested in
\[
 V_{\mu}(\bbeta)=\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bbeta\}^2 v_{\bar \btheta}(\X)+2l \EE_{\Ssc}\X\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bbeta\}v_{\bar \btheta}(\X)
\]
These to the new RWLS problem:
\[
\bar\bbeta={\rm argmin}_{\bbeta}V_{\mu}(\bbeta),\quad\mbox{s.t.}\quad\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha}|_{\bar\balpha}\bPsi\trans\bbeta=\bzero
\]
On the other hand, we need $\bar\bbeta=\bzero$ when the PS is correctly specified. It is obvious that when the PS is correctly specified, $l=0$. Hence, we only need to guarantee that 
\[
\bzero=\frac{\partial V_{\mu}(\bbeta)}{\partial\bbeta}\Big|_{\bbeta=0}=\EE_{\Ssc}\bPsi\exp(\X\trans\bar\bgamma)v_{\bar \btheta}(\X)=\EE_{\Tsc}\bPsi v_{\bar \btheta}(\X)
\]
so we can use the same $\bPsi$. 

For shortening the proof, we assume that 

Then we consider the asymptotic properties. We already have
\[
\muhat\subLAug=\widehat\EE_{\Ssc}(Y-\X\trans\balpha)\{\exp(\X\trans\widehat\bgamma)+\widehat\bPsi\trans\widehat\bbeta\}+\widehat\EE_{\Tsc}\X\trans\balpha.
\]
and $\mu_0:=\EE_{\Tsc}Y$. Let $\widetilde\mu\subLAug:=\widehat\EE_{\Ssc}(Y-\X\trans\balpha)\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bar\bbeta\}+\widehat\EE_{\Tsc}\X\trans\balpha$. By using Taylor series expansion, we have that
\begin{align*}
\muhat\subLAug-\widetilde\mu\subLAug&=n^{-1}\sum_{i=1}^n(Y_i-\X_i\trans\balpha)\{\exp(\X_i\trans\bar\bgamma)\X_i\trans(\widehat\bgamma-\bar\bgamma)+\bar\bbeta\trans(\widehat\bPsi-\bPsi)+\bPsi\trans(\widehat\bbeta-\bar\bbeta)\}+O_p(\bR)
\end{align*}
where $\bR$ represents the remainder and $O_p(\bR)=O_p(\left \| \widehat\bgamma-\bar\bgamma \right\|_2^2+\| \widehat\bPsi-\bPsi \|_2^2+ \| \widehat\bbeta-\bar\bbeta \|_2^2)$. The estimation $\widehat\bPsi$ has been given as $\widehat\bPsi=\bPhi-{\widehat\EE_{\Tsc}[\bPhi v_{\widehat\btheta}(\X)]}/{\widehat\EE_{\Tsc}v_{\widehat\btheta}(\X)}$, hence, we have
\[
\widehat\bPsi-\bPsi=\frac{\widehat\EE_{\Tsc}\{\bPhi v_{\widehat\btheta}(\X)\}}{\widehat\EE_{\Tsc}v_{\widehat\btheta}(\X)}-\frac{\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}}{\EE_{\Tsc} v_{\bar \btheta}(\X)}
\]
For shortening the proof, we assume that $v_{\widehat\btheta}(\X)=v_{\bar \btheta}(\X)=c$ for constant $c$, the variance of the residual is already known. Hence, by applying the central limit theorem, we have that
\begin{align*}
&\widehat\bPsi-\bPsi=\frac{\widehat\EE_{\Tsc}\{\bPhi v_{\bar \btheta}(\X)\}\EE_{\Tsc} v_{\bar \btheta}(\X)-\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}\widehat\EE_{\Tsc} v_{\bar \btheta}(\X)}{\widehat\EE_{\Tsc} v_{\bar \btheta}(\X)\EE_{\Tsc} v_{\bar \btheta}(\X)}
\\
&=\frac{\widehat\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}\EE_{\Tsc} v_{\bar \btheta}(\X)-\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}\EE_{\Tsc} v_{\bar \btheta}(\X)-[\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}\widehat\EE_{\Tsc} v_{\bar \btheta}(\X)-\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}\EE_{\Tsc} v_{\bar \btheta}(\X)]}{\{\EE_{\Tsc} v_{\bar \btheta}(\X)+O_p(n^{-1/2})\}\EE_{\Tsc} v_{\bar \btheta}(\X)}
\\
&=\frac{O_p(n^{-1/2})\EE_{\Tsc} v_{\bar \btheta}(\X)-\EE_{\Tsc}\{\bPhi  v_{\bar \btheta}(\X)\}O_p(n^{-1/2})}{\{\EE_{\Tsc} v_{\bar \btheta}(\X)+O_p(n^{-1/2})\}\EE_{\Tsc} v_{\bar \btheta}(\X)}=O_p(n^{-1/2})
\end{align*}

In addition, the estimation of $\bgamma$ has been given as
\[
\widehat\EE_{\Ssc}\X\exp(\X\trans\widehat\bgamma)=\widehat\EE_{\Tsc}\X
\]
by applying Taylor series expansion, we have
\[
n^{-1}\sum_{i=1}^n\X_i\exp(\X_i\trans\bar\bgamma)+n^{-1}\sum_{i=1}^n\X_i\exp(\X_i\trans\widetilde\bgamma)\X_i\trans(\widehat\bgamma-\bar\bgamma)=N^{-1}\sum_{i=n+1}^{n+N}\X_i
\]
where $\widetilde\bgamma$ is some vector between $\widehat\bgamma$ and $\bar\bgamma$. Let $\bJ$ represent matrix $n^{-1}\sum_{i=1}^n\X_i\exp(\X_i\trans\widetilde\bgamma)\X_i\trans$, which is obvious, a positive definite matrix. And we have
\begin{align*}
	\widehat\bgamma-\bar\bgamma=\bJ^{-1}\bigg\{N^{-1}\sum_{i=n+1}^{n+N}\X_i-n^{-1}\sum_{i=1}^n\X_i\exp(\X_i\trans\bar\bgamma)\bigg\}
\end{align*}
and we assume that $\frac{N}{n}\xrightarrow{} l$ where $l$ is a positive constant or $l=+\infty$. 

Next we consider the estimation of $\bbeta$. $\ba$, $\bb$ and $\bSigma$ can be estimated by $\widehat\ba:=\widehat\EE_{\Ssc}\widehat\bPsi\X\trans$, $\widehat\bb:=\widehat\EE_{\Ssc}\widehat\bPsi \exp(\X\trans\widehat\bgamma)v_{\widehat\btheta}(\X)$ and $\bSigmahat:=\widehat\EE_{\Ssc}\widehat\bPsi\widehat\bPsi\trans v_{\widehat\btheta}(\X)$. We already have that $\widehat\bPsi-\bPsi=O_p(n^{-1/2})$, and we get that
\[
\widehat\ba-\ba=\widehat\EE_{\Ssc}\widehat\bPsi\X\trans-\EE_{\Ssc}\bPsi\X\trans=\widehat\EE_{\Ssc}\bPsi\X\trans-\EE_{\Ssc}\bPsi\X\trans+O_p(n^{-1/2})=O_p(n^{-1/2})
\]
by using central limit theorem. Applying the same techniques, we have that $\widehat\bb-\bb=O_p(n^{-1/2})$ and $\bSigmahat-\bSigma=O_p(n^{-1/2})$. Furthermore, we can easily have that 
\begin{align*}
	\bSigmahat^{-1}-\bSigma^{-1}&=\bSigma^{-1}\bSigma\{\bSigma+O_p(n^{-1/2})\}^{-1}-\bSigma^{-1}
	\\&=\bSigma^{-1}[\bSigma\{\bSigma+O_p(n^{-1/2})\}^{-1}-\{\bSigma+O_p(n^{-1/2})\}\{\bSigma+O_p(n^{-1/2})\}^{-1}]
	\\&=O_p(n^{-1/2})
\end{align*}
based on which we can have $(\widehat\ba\trans\bSigmahat^{-1}\widehat\ba)^{-1}-(\ba\trans\bSigma^{-1}\ba)^{-1}=O_p(n^{-1/2})$ and then we can have $\bSigmahat^{-1}\widehat\ba(\widehat\ba\trans\bSigmahat^{-1}\widehat\ba)^{-1}\widehat\ba\trans\bSigmahat^{-1}-\bSigma^{-1}\ba(\ba\trans\bSigma^{-1}\ba)^{-1}\ba\trans\bSigma^{-1}=O_p(n^{-1/2})$ by using same techniques, hence, we have that
\begin{align*}
&\widehat\bbeta-\bar\bbeta=\bSigmahat^{-1}\widehat\ba(\widehat\ba\trans\bSigmahat^{-1}\widehat\ba)^{-1}\widehat\ba\trans\bSigmahat^{-1}\widehat\bb-\bSigmahat^{-1}\widehat\bb-\{\bSigma^{-1}\ba(\ba\trans\bSigma^{-1}\ba)^{-1}\ba\trans\bSigma^{-1}\bb-\bSigma^{-1}\bb\}
\\
&=\{\bSigma^{-1}\ba(\ba\trans\bSigma^{-1}\ba)^{-1}\ba\trans\bSigma^{-1}-\bSigma^{-1}\}(\widehat\bb-\bb)+\{\bSigmahat^{-1}\widehat\ba(\widehat\ba\trans\bSigmahat^{-1}\widehat\ba)^{-1}\widehat\ba\trans\bSigmahat^{-1}-\bSigma^{-1}\ba(\ba\trans\bSigma^{-1}\ba)^{-1}\ba\trans\bSigma^{-1}\}\widehat\bb
\\
&=\{\bSigma^{-1}\ba(\ba\trans\bSigma^{-1}\ba)^{-1}\ba\trans\bSigma^{-1}-\bSigma^{-1})O_p(n^{-1/2})+O_p(n^{-1/2}\}\{\bb+O_p(n^{-1/2})\}=O_p(n^{-1/2})
\end{align*}
thus by the definition of $\bR$, it is easy to notice that $O_p(\bR)=o_p(n^{-1/2})$. Assuming boundedness of the items, we have that
\begin{align*}
\muhat\subLAug-\widetilde\mu\subLAug=&n^{-1}\sum_{i=1}^n(Y_i-\bX_i\trans\balpha)\{\exp(\X_i\trans\bar\bgamma)\X_i\trans O_p(n^{-1/2})+\bar\bbeta\trans O_p(n^{-1/2})+\bPsi\trans O_p(n^{-1/2})\}+O_p(\bR)
\\=&O_p(n^{-1/2})+o_p(n^{-1/2})=O_p(n^{-1/2})
\end{align*}

When the OR: $m(\x)=\x\trans\balpha$ is correctly specified, we have 
\begin{align*}
	\EE(\widetilde\mu\subLAug)&=\EE[\widehat\EE_{\Ssc}(Y-\X\trans\balpha)\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bar\bbeta\}+\widehat\EE_{\Tsc}\X\trans\balpha]
	\\
	&=\EE_{\Ssc}(Y-\X\trans\balpha_0)\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bar\bbeta\}+\EE_{\Tsc}\X\trans\balpha_0
	\\
	&=\EE_{\Tsc}\X\trans\balpha_0=\EE_{\Tsc}Y=\mu_0
\end{align*}
Hence, by applying central limit theorem, we have  $n^{1/2}(\widetilde\mu\subLAug-\mu_0)$ weakly converges to gaussian distribution with mean $\bzero$. And we also have
\begin{align*}
    &\muhat\subLAug-\widetilde\mu\subLAug=n^{-1}\sum_{i=1}^n(Y_i-\X_i\trans\balpha_0)\{\exp(\X_i\trans\bar\bgamma)\X_i\trans(\widehat\bgamma-\bar\bgamma)+\bar\bbeta\trans(\widehat\bPsi-\bPsi)+\bPsi\trans(\widehat\bbeta-\bar\bbeta)\}+o_p(n^{-1/2})\\
    &=\bigg\{n^{-1}\sum_{i=1}^n(Y_i-\X_i\trans\balpha_0)\exp(\X_i\trans\bar\bgamma)\X_i\trans\bigg\}(\widehat\bgamma-\bar\bgamma)+n^{-1}\sum_{i=1}^n(Y_i-\X_i\trans\balpha_0)\{\bar\bbeta\trans(\widehat\bPsi-\bPsi)+\bPsi\trans(\widehat\bbeta-\bar\bbeta)\}
\end{align*}
It is obvious that $\EE_{\Ssc}(Y-\X\trans\balpha_0)=\EE_{\Ssc}(Y-\EE[Y\mid\X=\x])=0$ when OR is correctly specified. By using central limit theorem, $\muhat\subLAug-\widetilde\mu\subLAug=O_p(n^{-1/2})O_p(n^{-1/2})+O_p(n^{-1/2})O_p(n^{-1/2})+o_p(n^{-1/2})=o_p(n^{-1/2})$. Together with Slutsky theory we have that $\muhat\subLAug\xrightarrow{p}\mu_0$ and $n^{1/2}(\muhat\subLAug-\mu_0)$ weakly converges to gaussian distribution with mean $\bzero$. 

On the other hand, when the PS: $r(\x)=\exp(\x\trans\bar\bgamma)$ is correctly specified, $\bb=\EE_{\Ssc}\bPsi \exp(\X\trans\bgamma)v_{\bar \btheta}(\X)=\EE_{\Tsc}\bPsi v_{\bar \btheta}(\X)=0$ and thus $\bar\bbeta=\bzero$. We have that
\begin{align*}
    \EE(\widetilde\mu\subLAug)=&\EE[\widehat\EE_{\Ssc}(Y-\X\trans\balpha)\{\exp(\X\trans\bgamma_0)+\bPsi\trans\bar\bbeta\}+\widehat\EE_{\Tsc}\X\trans\balpha
\\=&\EE_{\Ssc}Y\exp(\X\trans\bgamma_0)-\EE_{\Ssc}\exp(\X\trans\bgamma_0)\X\trans\balpha_0+\EE_{\Tsc}\X\trans\balpha_0=\EE_{\Tsc}Y=\mu_0
\end{align*}
Hence, by applying central limit theorem, we have  $n^{1/2}(\widetilde\mu\subLAug-\mu_0)$ weakly converges to gaussian distribution with mean $\bzero$ and we have $\widetilde\mu\subLAug-\mu_0=O_p(n^{-1/2})$. On the other hand, we already have the asymptotic normal properties of $\widehat\bgamma$ and $\widehat\bPsi$. And it is worth noticing that $\bbeta$ is the function of $\bgamma$ and $\bPsi$. By Taylor series expansion and Slutsky theory, we have the asymptotic normality of $\widehat\bbeta$. Furthermore, we have that
\[
\muhat\subLAug-\widetilde\mu\subLAug=n^{-1}\sum_{i=1}^n(Y_i-\X_i\trans\balpha_0)\{\exp(\X_i\trans\bar\bgamma)\X_i\trans(\widehat\bgamma-\bar\bgamma)+\bPsi\trans(\widehat\bbeta-0)\}+o_p(n^{-1/2})=O_p(n^{-1/2})
\]
And we have $\muhat\subLAug-\mu_0=\muhat\subLAug-\widetilde\mu\subLAug+\widetilde\mu\subLAug-\mu_0=O_p(n^{-1/2})+O_p(n^{-1/2})=O_p(n^{-1/2})$ and $n^{1/2}(\muhat\subLAug-\mu_0)$ weakly converges to gaussian distribution with mean $\bzero$. 

$\EE_s\frac{\partial g(X\trans\alpha)}{\partial\alpha}|_{\widehat\alpha}\exp(X\trans\gamma_0)=\EE_T\frac{\partial g(X\trans\alpha)}{\partial\alpha}|_{\widehat\alpha}$

When the OR model is correct while the PS model is misspecified, the asymptotic variance of $\muhat\subLAug$ is $\Var(\widetilde\mu\subLAug)=\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bar\bbeta\}^2 v_{\bar \btheta}(\X)+\Var_{\Tsc}(\X\trans\balpha)$ and $\bar\bbeta$ is designed to minimize the variance. It is worth notice that when $\bar\bbeta=\bzero$, $\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bar\bbeta\}^2 v_{\bar \btheta}(\X)+\Var_{\Tsc}(\X\trans\balpha)=\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)\}^2 v_{\bar \btheta}(\X)+\Var_{\Tsc}(\X\trans\balpha)$, which is the asymptotic variance of $\muhat\subCB$. Hence, By the definition of $\bar\bbeta$, we have that $\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)+\bPsi\trans\bar\bbeta\}^2 v_{\bar \btheta}(\X)\leq\EE_{\Ssc}\{\exp(\X\trans\bar\bgamma)\}^2 v_{\bar \btheta}(\X)$, and when $\bar\bbeta\neq 0$, $\muhat\subLAug$ has a smaller asymptotic variance than $\muhat\subCB$.

On the other hand, when $\bar\bgamma=\bgamma_0$, we already have $\widehat\bgamma-\bar\bgamma=O_p(n^{-1/2})$. Hence, we have that 
\begin{align*}
\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\widehat\balpha}\exp(\X\trans\bgamma_0)-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\widehat\balpha}
&=\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\bar\balpha}\exp(\X\trans\bgamma_0)-\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\bar\balpha}\exp(\X\trans\bgamma_0)\\
&+\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\bar\balpha}-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\bar\balpha}+o_p(n^{-1/2})=O_p(n^{-1/2})
\end{align*}
by using central limit theorem. And we further have
\begin{align*}
    \widehat\bL=\bigg\{\widehat\EE_{\Ssc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\widehat\balpha}\exp(\X\trans\bgamma_0)-\widehat\EE_{\Tsc}\frac{\partial g(\X\trans\balpha)}{\partial \balpha\trans}\bigg|_{\widehat\balpha}\bigg\}\EE_{\Ssc}\bigg\{\frac{\partial S(\balpha)}{\partial \balpha\trans}\bigg|_{\balpha}\bigg\}^{-1}+O_p(n^{-1/2})=O_p(n^{-1/2}).
\end{align*}
In addition, we also have that $\widehat\EE_{\Ssc}\widehat\bPsi \exp(\X\trans\widehat\bgamma)v_{\widehat\btheta}(\X)=\widehat\EE_{\Ssc}\bPsi \exp(\X\trans\bar\bgamma)v_{\bar\btheta}(\X)+O_p(n^{-1/2})=O_p(n^{-1/2})$. Thus, it is obvious that $\widehat\bbeta=\widehat\bOmega\widehat\bb=\{\bOmega+o_p(1)\}O_p(n^{-1/2})=O_p(n^{-1/2})$.

